Robust Partial-to-Partial Point Cloud Registration in a Full Range

Point cloud registration for 3D objects is a challenging task due to sparse and noisy measurements, incomplete observations and large transformations. In this work, we propose \textbf{G}raph \textbf{M}atching \textbf{C}onsensus \textbf{Net}work (\textbf{GMCNet}), which estimates pose-invariant correspondences for full-range Partial-to-Partial point cloud Registration (PPR) in the object-level registration scenario. To encode robust point descriptors, \textbf{1)} we first comprehensively investigate transformation-robustness and noise-resilience of various geometric features. \textbf{2)} Then, we employ a novel {T}ransformation-robust {P}oint {T}ransformer (\textbf{TPT}) module to adaptively aggregate local features regarding the structural relations, which takes advantage from both handcrafted rotation-invariant ({\textit{RI}}) features and noise-resilient spatial coordinates. \textbf{3)} Based on a synergy of hierarchical graph networks and graphical modeling, we propose the {H}ierarchical {G}raphical {M}odeling (\textbf{HGM}) architecture to encode robust descriptors consisting of i) a unary term learned from {\textit{RI}} features; and ii) multiple smoothness terms encoded from neighboring point relations at different scales through our TPT modules. Moreover, we construct a challenging PPR dataset (\textbf{MVP-RG}) based on the recent MVP dataset that features high-quality scans. Extensive experiments show that GMCNet outperforms previous state-of-the-art methods for PPR. Notably, GMCNet encodes point descriptors for each point cloud individually without using cross-contextual information, or ground truth correspondences for training. Our code and datasets are available at: https://github.com/paul007pl/GMCNet.

==> table/mn40.tex <==
{\setlength{\tabcolsep}{3pt}
\begin{table*}[]
    % \centering
    \caption{
    \textbf{PPR on ModelNet40.} 
    $^{\dag}$ denotes ground truth correspondences or cross-contextual information are used during training.
    }
    \vspace{-2mm}
    \begin{center}
    \small{
        \begin{tabular}{l|ccc|ccc||ccc|ccc||ccc|ccc}
            % \Xhline{1pt}
            \toprule[1.2pt]
            \multicolumn{1}{c}{\multirow{3}{*}{}} & \multicolumn{6}{c||}{Clean} & \multicolumn{6}{c||}{Unseen} & \multicolumn{6}{c}{Noise}  \\
            \cline{2-19}
            \multicolumn{1}{c}{} 
            & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c||}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}}
            & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c||}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}}
            & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}}
            \\
            \cline{2-19}
            \multicolumn{1}{c}{} & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$
              
            & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$
             
            & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$
            \\
            % \hline\hline
            \midrule[0.75pt]\midrule[0.75pt]
            \scriptsize PRNet$^{\dag}$~\citep{wang2019prnet} & \fontsize{6}{6}\selectfont 8.00\textdegree & \fontsize{6}{6}\selectfont 0.054 & \fontsize{6}{6}\selectfont 0.073 &  \fontsize{6}{6}\selectfont 98.16\textdegree & \fontsize{6}{6}\selectfont 0.325 & \fontsize{6}{6}\selectfont 0.543 &
            \fontsize{6}{6}\selectfont 3.19\textdegree & \fontsize{6}{6}\selectfont 0.028 & \fontsize{6}{6}\selectfont 0.036 &  \fontsize{6}{6}\selectfont 91.94\textdegree & \fontsize{6}{6}\selectfont 0.297 & \fontsize{6}{6}\selectfont 0.545 &
            \fontsize{6}{6}\selectfont 4.37\textdegree & \fontsize{6}{6}\selectfont 0.034 & \fontsize{6}{6}\selectfont 0.045 & \fontsize{6}{6}\selectfont 95.80\textdegree & \fontsize{6}{6}\selectfont 0.319 & \fontsize{6}{6}\selectfont 0.542 
              \\
            \scriptsize IDAM$^{\dag}$({GNN})~\citep{li2019iterative}& \fontsize{6}{6}\selectfont 1.66\textdegree & \fontsize{6}{6}\selectfont 0.009 & \fontsize{6}{6}\selectfont 0.013 & \fontsize{6}{6}\selectfont 25.36\textdegree & \fontsize{6}{6}\selectfont 0.126 & \fontsize{6}{6}\selectfont 0.166 &
            \fontsize{6}{6}\selectfont 1.61\textdegree & \fontsize{6}{6}\selectfont 0.010 & \fontsize{6}{6}\selectfont 0.014 & \fontsize{6}{6}\selectfont 20.80\textdegree & \fontsize{6}{6}\selectfont 0.112 & \fontsize{6}{6}\selectfont 0.146 &
            \fontsize{6}{6}\selectfont 4.46\textdegree & \fontsize{6}{6}\selectfont 0.029 & \fontsize{6}{6}\selectfont 0.039 & \fontsize{6}{6}\selectfont 57.85\textdegree & \fontsize{6}{6}\selectfont 0.253 & \fontsize{6}{6}\selectfont 0.374
             \\
            \scriptsize IDAM$^{\dag}$(\textit{FPFH})~\citep{li2019iterative} & \fontsize{6}{6}\selectfont 0.93\textdegree & \fontsize{6}{6}\selectfont 0.005 & \fontsize{6}{6}\selectfont 0.007 & \fontsize{6}{6}\selectfont 18.06\textdegree & \fontsize{6}{6}\selectfont 0.083 & \fontsize{6}{6}\selectfont 0.115 &
            \fontsize{6}{6}\selectfont 0.86\textdegree & \fontsize{6}{6}\selectfont 0.005 & \fontsize{6}{6}\selectfont 0.007 & \fontsize{6}{6}\selectfont 16.17\textdegree & \fontsize{6}{6}\selectfont 0.073 & \fontsize{6}{6}\selectfont 0.106 &
            \fontsize{6}{6}\selectfont 9.60\textdegree & \fontsize{6}{6}\selectfont 0.052 & \fontsize{6}{6}\selectfont 0.084 & \fontsize{6}{6}\selectfont 71.06\textdegree & \fontsize{6}{6}\selectfont 0.217 & \fontsize{6}{6}\selectfont 0.430 
             \\
            \scriptsize RGM$^{\dag}$~\citep{fu2021robust} & \fontsize{6}{6}\selectfont 0.30\textdegree & \fontsize{6}{6}\selectfont 0.002 & \fontsize{6}{6}\selectfont 0.003 & \fontsize{6}{6}\selectfont 24.10\textdegree & \fontsize{6}{6}\selectfont 0.115 & \fontsize{6}{6}\selectfont 0.160 &
            \fontsize{6}{6}\selectfont 0.34\textdegree & \fontsize{6}{6}\selectfont 0.004 & \fontsize{6}{6}\selectfont 0.004 & \fontsize{6}{6}\selectfont 8.78\textdegree & \fontsize{6}{6}\selectfont 0.076 & \fontsize{6}{6}\selectfont 0.084 &
            \fontsize{6}{6}\selectfont 2.21\textdegree & \fontsize{6}{6}\selectfont 0.013 & \fontsize{6}{6}\selectfont 0.018 & \fontsize{6}{6}\selectfont 23.58\textdegree & \fontsize{6}{6}\selectfont 0.111 & \fontsize{6}{6}\selectfont 0.156
             \\
            \scriptsize Predator$^{\dag}$~\citep{huang2021predator} & \fontsize{6}{6}\selectfont 1.60\textdegree & \fontsize{6}{6}\selectfont 0.012 & \fontsize{6}{6}\selectfont 0.015 & \fontsize{6}{6}\selectfont 15.33\textdegree & \fontsize{6}{6}\selectfont 0.041 & \fontsize{6}{6}\selectfont 0.077 &
            \fontsize{6}{6}\selectfont 1.32\textdegree & \fontsize{6}{6}\selectfont 0.009 & \fontsize{6}{6}\selectfont 0.012 & \fontsize{6}{6}\selectfont 11.59\textdegree & \fontsize{6}{6}\selectfont 0.032 & \fontsize{6}{6}\selectfont 0.058 & 
            \fontsize{6}{6}\selectfont 3.33\textdegree & \fontsize{6}{6}\selectfont 0.018 & \fontsize{6}{6}\selectfont 0.026 & \fontsize{6}{6}\selectfont 40.64\textdegree & \fontsize{6}{6}\selectfont 0.110 & \fontsize{6}{6}\selectfont 0.207 \\
            \hline
            \scriptsize DCP~\citep{wang2019deep} & \fontsize{6}{6}\selectfont 10.24\textdegree & \fontsize{6}{6}\selectfont 0.071 & \fontsize{6}{6}\selectfont 0.103 &  \fontsize{6}{6}\selectfont 70.51\textdegree & \fontsize{6}{6}\selectfont 0.186 & \fontsize{6}{6}\selectfont 0.425 &
            \fontsize{6}{6}\selectfont 11.92\textdegree & \fontsize{6}{6}\selectfont 0.076 & \fontsize{6}{6}\selectfont 0.119 &  \fontsize{6}{6}\selectfont 67.39\textdegree & \fontsize{6}{6}\selectfont 0.170 & \fontsize{6}{6}\selectfont 0.410 &
            \fontsize{6}{6}\selectfont 9.33\textdegree & \fontsize{6}{6}\selectfont 0.070 & \fontsize{6}{6}\selectfont 0.097 & \fontsize{6}{6}\selectfont 73.61\textdegree & \fontsize{6}{6}\selectfont 0.185 & \fontsize{6}{6}\selectfont 0.441
             \\
            \scriptsize DeepGMR (\textit{RRI})~\citep{yuan2020deepgmr} & \fontsize{6}{6}\selectfont 16.95\textdegree & \fontsize{6}{6}\selectfont 0.070 & \fontsize{6}{6}\selectfont 0.122 &  \fontsize{6}{6}\selectfont 45.38\textdegree & \fontsize{6}{6}\selectfont 0.210 & \fontsize{6}{6}\selectfont 0.321 &
            \fontsize{6}{6}\selectfont 17.45\textdegree & \fontsize{6}{6}\selectfont 0.074 & \fontsize{6}{6}\selectfont 0.130 & \fontsize{6}{6}\selectfont 49.23\textdegree & \fontsize{6}{6}\selectfont 0.219 & \fontsize{6}{6}\selectfont 0.349 &
            \fontsize{6}{6}\selectfont 16.96\textdegree & \fontsize{6}{6}\selectfont 0.068 & \fontsize{6}{6}\selectfont 0.120 & \fontsize{6}{6}\selectfont 68.68\textdegree & \fontsize{6}{6}\selectfont 0.248 & \fontsize{6}{6}\selectfont 0.419 
              \\
            \scriptsize DeepGMR (Pts)~\citep{yuan2020deepgmr} & \fontsize{6}{6}\selectfont 6.60\textdegree & \fontsize{6}{6}\selectfont 0.050 & \fontsize{6}{6}\selectfont 0.065 & \fontsize{6}{6}\selectfont 67.81\textdegree & \fontsize{6}{6}\selectfont 0.244 & \fontsize{6}{6}\selectfont 0.416 &
            \fontsize{6}{6}\selectfont 8.05\textdegree & \fontsize{6}{6}\selectfont 0.053 & \fontsize{6}{6}\selectfont 0.074 & \fontsize{6}{6}\selectfont 72.27\textdegree & \fontsize{6}{6}\selectfont 0.245 & \fontsize{6}{6}\selectfont 0.449 &
            \fontsize{6}{6}\selectfont 6.48\textdegree & \fontsize{6}{6}\selectfont 0.049 & \fontsize{6}{6}\selectfont 0.064 & \fontsize{6}{6}\selectfont 70.26\textdegree & \fontsize{6}{6}\selectfont 0.246 & \fontsize{6}{6}\selectfont 0.428 
              \\
            \scriptsize RPMNet (\textit{PPF})~\citep{yew2020rpm} & \fontsize{6}{6}\selectfont 0.78\textdegree & \fontsize{6}{6}\selectfont 0.005 & \fontsize{6}{6}\selectfont 0.006 & \fontsize{6}{6}\selectfont 15.84\textdegree & \fontsize{6}{6}\selectfont 0.070 & \fontsize{6}{6}\selectfont 0.098 &
            \fontsize{6}{6}\selectfont 0.60\textdegree & \fontsize{6}{6}\selectfont 0.004 & \fontsize{6}{6}\selectfont 0.005 & \fontsize{6}{6}\selectfont 16.91\textdegree & \fontsize{6}{6}\selectfont 0.079 & \fontsize{6}{6}\selectfont 0.127 &
            \fontsize{6}{6}\selectfont 3.52\textdegree & \fontsize{6}{6}\selectfont 0.214 & \fontsize{6}{6}\selectfont 0.029 & \fontsize{6}{6}\selectfont 37.82\textdegree & \fontsize{6}{6}\selectfont 0.132 & \fontsize{6}{6}\selectfont 0.250  
              \\
            \hline
            \scriptsize \OM{} (\textit{RRI})  & \fontsize{6}{6}\selectfont 0.013\textdegree & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont \textbf{0.036\textdegree} & \fontsize{6}{6}\selectfont \textbf{0.0002} & \fontsize{6}{6}\selectfont \textbf{0.0002} &
            \fontsize{6}{6}\selectfont 0.017\textdegree & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont \textbf{0.053\textdegree} & \fontsize{6}{6}\selectfont \textbf{0.0004} & \fontsize{6}{6}\selectfont \textbf{0.0005} &
            \fontsize{6}{6}\selectfont 1.28\textdegree & \fontsize{6}{6}\selectfont 0.009 & \fontsize{6}{6}\selectfont 0.011 & \fontsize{6}{6}\selectfont 50.62\textdegree & \fontsize{6}{6}\selectfont 0.206 & \fontsize{6}{6}\selectfont 0.315 \\
            \scriptsize \OM{} (\textit{FPFH})  & \fontsize{6}{6}\selectfont \textbf{0.012\textdegree} & \fontsize{6}{6}\selectfont \textbf{\textless 0.0001} & \fontsize{6}{6}\selectfont \textbf{\textless 0.0001} & \fontsize{6}{6}\selectfont 0.253\textdegree & \fontsize{6}{6}\selectfont 0.0008 & \fontsize{6}{6}\selectfont 0.0016 &
            \fontsize{6}{6}\selectfont \textbf{0.014\textdegree} & \fontsize{6}{6}\selectfont \textbf{\textless 0.0001} & \fontsize{6}{6}\selectfont \textbf{\textless 0.0001} & \fontsize{6}{6}\selectfont 0.549\textdegree & \fontsize{6}{6}\selectfont 0.0024 & \fontsize{6}{6}\selectfont 0.0033 & 
            \fontsize{6}{6}\selectfont 1.18\textdegree & \fontsize{6}{6}\selectfont 0.008 & \fontsize{6}{6}\selectfont 0.010 & \fontsize{6}{6}\selectfont 25.95\textdegree & \fontsize{6}{6}\selectfont 0.115 & \fontsize{6}{6}\selectfont 0.184 \\
            \scriptsize \OM{} (\textit{PPF})  & \fontsize{6}{6}\selectfont 0.016\textdegree & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont \textless 0.0001 & \fontsize{6}{6}\selectfont 0.284\textdegree & \fontsize{6}{6}\selectfont 0.0011 & \fontsize{6}{6}\selectfont 0.0017 &
            \fontsize{6}{6}\selectfont 0.026\textdegree & \fontsize{6}{6}\selectfont 0.0002 & \fontsize{6}{6}\selectfont 0.0002 & \fontsize{6}{6}\selectfont 0.388\textdegree & \fontsize{6}{6}\selectfont 0.0024 & \fontsize{6}{6}\selectfont 0.0030 & 
            \fontsize{6}{6}\selectfont \textbf{0.94\textdegree} & \fontsize{6}{6}\selectfont \textbf{0.007} & \fontsize{6}{6}\selectfont \textbf{0.008} & \fontsize{6}{6}\selectfont \textbf{18.13\textdegree} & \fontsize{6}{6}\selectfont \textbf{0.093} & \fontsize{6}{6}\selectfont \textbf{0.132} \\
            % \Xhline{1pt}
            \bottomrule[1.2pt]
        \end{tabular}
    }
    \end{center}
    \label{tab:mn40}
\end{table*}
}

==> table/mn40_clean.tex <==
\begin{table}[]
    \setlength{\tabcolsep}{5.5pt}
    \caption{
    \textbf{PPR on ModelNet40 (Clean).} 
    $^{\dag}$ denotes ground truth correspondences or cross-contextual information are used during training.
    }
    \begin{center}
        \begin{tabular}{l|ccc|ccc}
            \toprule[1.2pt]
            % \toprule\setlength{\heavyrulewidth}{1.2pt}
            % \toprule
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}} \\
            % \cline{2-7}
            \cmidrule[0.25pt]{2-7}
            % \cmidrule{2-7}
            \multicolumn{1}{c}{} & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$ \\
            % \midrule[0.5pt]\midrule[0.5pt] 
            \midrule[0.75pt] 
            % \midrule
            \scriptsize PRNet$^{\dag}$~\citep{wang2019prnet} & \fontsize{6.5}{6.5}\selectfont 8.00\textdegree & \fontsize{6.5}{6.5}\selectfont 0.054 & \fontsize{6.5}{6.5}\selectfont 0.073 &  \fontsize{6.5}{6.5}\selectfont 98.16\textdegree & \fontsize{6.5}{6.5}\selectfont 0.325 & \fontsize{6.5}{6.5}\selectfont 0.543 \\
            \scriptsize IDAM$^{\dag}$({GNN})~\citep{li2019iterative}& \fontsize{6.5}{6.5}\selectfont 1.66\textdegree & \fontsize{6.5}{6.5}\selectfont 0.009 & \fontsize{6.5}{6.5}\selectfont 0.013 & \fontsize{6.5}{6.5}\selectfont 25.36\textdegree & \fontsize{6.5}{6.5}\selectfont 0.126 & \fontsize{6.5}{6.5}\selectfont 0.166 \\
            \scriptsize IDAM$^{\dag}$(\textit{FPFH})~\citep{li2019iterative} & \fontsize{6.5}{6.5}\selectfont 0.93\textdegree & \fontsize{6.5}{6.5}\selectfont 0.005 & \fontsize{6.5}{6.5}\selectfont 0.007 & \fontsize{6.5}{6.5}\selectfont 18.06\textdegree & \fontsize{6.5}{6.5}\selectfont 0.083 & \fontsize{6.5}{6.5}\selectfont 0.115 \\
            \scriptsize RGM$^{\dag}$~\citep{fu2021robust} & \fontsize{6.5}{6.5}\selectfont 0.30\textdegree & \fontsize{6.5}{6.5}\selectfont 0.002 & \fontsize{6.5}{6.5}\selectfont 0.003 & \fontsize{6.5}{6.5}\selectfont 24.10\textdegree & \fontsize{6.5}{6.5}\selectfont 0.115 & \fontsize{6.5}{6.5}\selectfont 0.160 \\
            \scriptsize Predator$^{\dag}$~\citep{huang2021predator} & \fontsize{6.5}{6.5}\selectfont 1.60\textdegree & \fontsize{6.5}{6.5}\selectfont 0.012 & \fontsize{6.5}{6.5}\selectfont 0.015 & \fontsize{6.5}{6.5}\selectfont 15.33\textdegree & \fontsize{6.5}{6.5}\selectfont 0.041 & \fontsize{6.5}{6.5}\selectfont 0.077 \\
            \scriptsize DCP~\citep{wang2019deep} & \fontsize{6.5}{6.5}\selectfont 10.24\textdegree & \fontsize{6.5}{6.5}\selectfont 0.071 & \fontsize{6.5}{6.5}\selectfont 0.103 &  \fontsize{6.5}{6.5}\selectfont 70.51\textdegree & \fontsize{6.5}{6.5}\selectfont 0.186 & \fontsize{6.5}{6.5}\selectfont 0.425 \\
            \scriptsize DeepGMR (\textit{RRI})~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 16.95\textdegree & \fontsize{6.5}{6.5}\selectfont 0.070 & \fontsize{6.5}{6.5}\selectfont 0.122 &  \fontsize{6.5}{6.5}\selectfont 45.38\textdegree & \fontsize{6.5}{6.5}\selectfont 0.210 & \fontsize{6.5}{6.5}\selectfont 0.321 \\
            \scriptsize DeepGMR (XYZ)~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 6.60\textdegree & \fontsize{6.5}{6.5}\selectfont 0.050 & \fontsize{6.5}{6.5}\selectfont 0.065 & \fontsize{6.5}{6.5}\selectfont 67.81\textdegree & \fontsize{6.5}{6.5}\selectfont 0.244 & \fontsize{6.5}{6.5}\selectfont 0.416 \\
            \scriptsize RPMNet (\textit{PPF})~\citep{yew2020rpm} & \fontsize{6.5}{6.5}\selectfont 0.78\textdegree & \fontsize{6.5}{6.5}\selectfont 0.005 & \fontsize{6.5}{6.5}\selectfont 0.006 & \fontsize{6.5}{6.5}\selectfont 15.84\textdegree & \fontsize{6.5}{6.5}\selectfont 0.070 & \fontsize{6.5}{6.5}\selectfont 0.098 \\
            \midrule[0.25pt]
            % \midrule
            \scriptsize \OM{} (\textit{RRI})  & \fontsize{6.5}{6.5}\selectfont 0.013\textdegree & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont \textbf{0.036\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{0.0002} & \fontsize{6.5}{6.5}\selectfont \textbf{0.0002} \\
            \scriptsize \OM{} (\textit{FPFH})  & \fontsize{6.5}{6.5}\selectfont \textbf{0.012\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{\textless 0.0001} & \fontsize{6.5}{6.5}\selectfont \textbf{\textless 0.0001} & \fontsize{6.5}{6.5}\selectfont 0.253\textdegree & \fontsize{6.5}{6.5}\selectfont 0.0008 & \fontsize{6.5}{6.5}\selectfont 0.0016 \\
            \scriptsize \OM{} (\textit{PPF})  & \fontsize{6.5}{6.5}\selectfont 0.016\textdegree & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont 0.284\textdegree & \fontsize{6.5}{6.5}\selectfont 0.0011 & \fontsize{6.5}{6.5}\selectfont 0.0017 \\
            \bottomrule[1.2pt]
            % \bottomrule
        \end{tabular}
    \end{center}
    \label{tab:mn40_clean}
\end{table}

==> table/mn40_noisy.tex <==
\begin{table}[]
    \setlength{\tabcolsep}{5.5pt}
    \caption{
    \textbf{PPR on ModelNet40 (Noisy).} 
    $^{\dag}$ denotes ground truth correspondences or cross-contextual information are used during training.
    }
    \begin{center}
        \begin{tabular}{l|ccc|ccc}
            \toprule[1.2pt]
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}} \\
            % \cline{2-7}
            \cmidrule[0.25pt]{2-7}
            \multicolumn{1}{c}{} & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$ \\
            % \midrule[0.5pt]\midrule[0.5pt] 
            \midrule[0.75pt] 
            \scriptsize PRNet$^{\dag}$~\citep{wang2019prnet} & \fontsize{6.5}{6.5}\selectfont 4.37\textdegree & \fontsize{6.5}{6.5}\selectfont 0.034 & \fontsize{6.5}{6.5}\selectfont 0.045 & \fontsize{6.5}{6.5}\selectfont 95.80\textdegree & \fontsize{6.5}{6.5}\selectfont 0.319 & \fontsize{6.5}{6.5}\selectfont 0.542  \\
            \scriptsize IDAM$^{\dag}$({GNN})~\citep{li2019iterative}& \fontsize{6.5}{6.5}\selectfont 4.46\textdegree & \fontsize{6.5}{6.5}\selectfont 0.029 & \fontsize{6.5}{6.5}\selectfont 0.039 & \fontsize{6.5}{6.5}\selectfont 57.85\textdegree & \fontsize{6.5}{6.5}\selectfont 0.253 & \fontsize{6.5}{6.5}\selectfont 0.374 \\
            \scriptsize IDAM$^{\dag}$(\textit{FPFH})~\citep{li2019iterative} & \fontsize{6.5}{6.5}\selectfont 9.60\textdegree & \fontsize{6.5}{6.5}\selectfont 0.052 & \fontsize{6.5}{6.5}\selectfont 0.084 & \fontsize{6.5}{6.5}\selectfont 71.06\textdegree & \fontsize{6.5}{6.5}\selectfont 0.217 & \fontsize{6.5}{6.5}\selectfont 0.430 \\
            \scriptsize RGM$^{\dag}$~\citep{fu2021robust} & \fontsize{6.5}{6.5}\selectfont 2.21\textdegree & \fontsize{6.5}{6.5}\selectfont 0.013 & \fontsize{6.5}{6.5}\selectfont 0.018 & \fontsize{6.5}{6.5}\selectfont 23.58\textdegree & \fontsize{6.5}{6.5}\selectfont 0.111 & \fontsize{6.5}{6.5}\selectfont 0.156 \\
            \scriptsize Predator$^{\dag}$~\citep{huang2021predator} & \fontsize{6.5}{6.5}\selectfont 3.33\textdegree & \fontsize{6.5}{6.5}\selectfont 0.018 & \fontsize{6.5}{6.5}\selectfont 0.026 & \fontsize{6.5}{6.5}\selectfont 40.64\textdegree & \fontsize{6.5}{6.5}\selectfont 0.110 & \fontsize{6.5}{6.5}\selectfont 0.207 \\
            \scriptsize DCP~\citep{wang2019deep} & \fontsize{6.5}{6.5}\selectfont 9.33\textdegree & \fontsize{6.5}{6.5}\selectfont 0.070 & \fontsize{6.5}{6.5}\selectfont 0.097 & \fontsize{6.5}{6.5}\selectfont 73.61\textdegree & \fontsize{6.5}{6.5}\selectfont 0.185 & \fontsize{6.5}{6.5}\selectfont 0.441 \\
            \scriptsize DeepGMR (\textit{RRI})~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 16.96\textdegree & \fontsize{6.5}{6.5}\selectfont 0.068 & \fontsize{6.5}{6.5}\selectfont 0.120 & \fontsize{6.5}{6.5}\selectfont 68.68\textdegree & \fontsize{6.5}{6.5}\selectfont 0.248 & \fontsize{6.5}{6.5}\selectfont 0.419 \\
            \scriptsize DeepGMR (XYZ)~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 6.48\textdegree & \fontsize{6.5}{6.5}\selectfont 0.049 & \fontsize{6.5}{6.5}\selectfont 0.064 & \fontsize{6.5}{6.5}\selectfont 70.26\textdegree & \fontsize{6.5}{6.5}\selectfont 0.246 & \fontsize{6.5}{6.5}\selectfont 0.428 \\
            \scriptsize RPMNet (\textit{PPF})~\citep{yew2020rpm} & \fontsize{6.5}{6.5}\selectfont 3.52\textdegree & \fontsize{6.5}{6.5}\selectfont 0.214 & \fontsize{6.5}{6.5}\selectfont 0.029 & \fontsize{6.5}{6.5}\selectfont 37.82\textdegree & \fontsize{6.5}{6.5}\selectfont 0.132 & \fontsize{6.5}{6.5}\selectfont 0.250 \\
            \midrule[0.25pt]
            \scriptsize \OM{} (\textit{RRI})  & \fontsize{6.5}{6.5}\selectfont 1.28\textdegree & \fontsize{6.5}{6.5}\selectfont 0.009 & \fontsize{6.5}{6.5}\selectfont 0.011 & \fontsize{6.5}{6.5}\selectfont 50.62\textdegree & \fontsize{6.5}{6.5}\selectfont 0.206 & \fontsize{6.5}{6.5}\selectfont 0.315 \\
            \scriptsize \OM{} (\textit{FPFH})  & \fontsize{6.5}{6.5}\selectfont 1.18\textdegree & \fontsize{6.5}{6.5}\selectfont 0.008 & \fontsize{6.5}{6.5}\selectfont 0.010 & \fontsize{6.5}{6.5}\selectfont 25.95\textdegree & \fontsize{6.5}{6.5}\selectfont 0.115 & \fontsize{6.5}{6.5}\selectfont 0.184  \\
            \scriptsize \OM{} (\textit{PPF})  & \fontsize{6.5}{6.5}\selectfont \textbf{0.94\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{0.007} & \fontsize{6.5}{6.5}\selectfont \textbf{0.008} &
            \fontsize{6.5}{6.5}\selectfont \textbf{18.13\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{0.093} & \fontsize{6.5}{6.5}\selectfont \textbf{0.132} \\
            \bottomrule[1.2pt]
        \end{tabular}
    \end{center}
    \label{tab:mn40_noisy}
\end{table}

==> table/mn40_unseen.tex <==
\begin{table}[]
    \setlength{\tabcolsep}{4.5pt}
    \caption{
    \textbf{PPR on ModelNet40 (Unseen).} 
    $^{\dag}$ denotes ground truth correspondences or cross-contextual information are used during training.
    }
    \begin{center}
        \begin{tabular}{l|ccc|ccc}
            \toprule[1.2pt]
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}} \\
            % \cline{2-7}
            \cmidrule[0.25pt]{2-7}
            \multicolumn{1}{c}{} & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$   & \scriptsize $\mathcal{L}_{\mathbf{R}}$   & \scriptsize $\mathcal{L}_{\mathbf{t}}$   & \scriptsize $\mathcal{L}_{\text{RMSE}}$ \\
            % \midrule[0.5pt]\midrule[0.5pt] 
            \midrule[0.75pt]
            \scriptsize PRNet$^{\dag}$~\citep{wang2019prnet} & \fontsize{6.5}{6.5}\selectfont 3.19\textdegree & \fontsize{6.5}{6.5}\selectfont 0.028 & \fontsize{6.5}{6.5}\selectfont 0.036 &  \fontsize{6.5}{6.5}\selectfont 91.94\textdegree & \fontsize{6.5}{6.5}\selectfont 0.297 & \fontsize{6.5}{6.5}\selectfont 0.545 \\
            \scriptsize IDAM$^{\dag}$({GNN})~\citep{li2019iterative}& \fontsize{6.5}{6.5}\selectfont 1.61\textdegree & \fontsize{6.5}{6.5}\selectfont 0.010 & \fontsize{6.5}{6.5}\selectfont 0.014 & \fontsize{6.5}{6.5}\selectfont 20.80\textdegree & \fontsize{6.5}{6.5}\selectfont 0.112 & \fontsize{6.5}{6.5}\selectfont 0.146 \\
            \scriptsize IDAM$^{\dag}$(\textit{FPFH})~\citep{li2019iterative} & \fontsize{6.5}{6.5}\selectfont 0.86\textdegree & \fontsize{6.5}{6.5}\selectfont 0.005 & \fontsize{6.5}{6.5}\selectfont 0.007 & \fontsize{6.5}{6.5}\selectfont 16.17\textdegree & \fontsize{6.5}{6.5}\selectfont 0.073 & \fontsize{6.5}{6.5}\selectfont 0.106 \\
            \scriptsize RGM$^{\dag}$~\citep{fu2021robust} & \fontsize{6.5}{6.5}\selectfont 0.34\textdegree & \fontsize{6.5}{6.5}\selectfont 0.004 & \fontsize{6.5}{6.5}\selectfont 0.004 & \fontsize{6.5}{6.5}\selectfont 8.78\textdegree & \fontsize{6.5}{6.5}\selectfont 0.076 & \fontsize{6.5}{6.5}\selectfont 0.084 \\
            \scriptsize Predator$^{\dag}$~\citep{huang2021predator} & \fontsize{6.5}{6.5}\selectfont 1.32\textdegree & \fontsize{6.5}{6.5}\selectfont 0.009 & \fontsize{6.5}{6.5}\selectfont 0.012 & \fontsize{6.5}{6.5}\selectfont 11.59\textdegree & \fontsize{6.5}{6.5}\selectfont 0.032 & \fontsize{6.5}{6.5}\selectfont 0.058 \\
            \scriptsize DCP~\citep{wang2019deep} & \fontsize{6.5}{6.5}\selectfont 11.92\textdegree & \fontsize{6.5}{6.5}\selectfont 0.076 & \fontsize{6.5}{6.5}\selectfont 0.119 &  \fontsize{6.5}{6.5}\selectfont 67.39\textdegree & \fontsize{6.5}{6.5}\selectfont 0.170 & \fontsize{6.5}{6.5}\selectfont 0.410 \\
            \scriptsize DeepGMR (\textit{RRI})~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 17.45\textdegree & \fontsize{6.5}{6.5}\selectfont 0.074 & \fontsize{6.5}{6.5}\selectfont 0.130 & \fontsize{6.5}{6.5}\selectfont 49.23\textdegree & \fontsize{6.5}{6.5}\selectfont 0.219 & \fontsize{6.5}{6.5}\selectfont 0.349 \\
            \scriptsize DeepGMR (XYZ)~\citep{yuan2020deepgmr} & \fontsize{6.5}{6.5}\selectfont 8.05\textdegree & \fontsize{6.5}{6.5}\selectfont 0.053 & \fontsize{6.5}{6.5}\selectfont 0.074 & \fontsize{6.5}{6.5}\selectfont 72.27\textdegree & \fontsize{6.5}{6.5}\selectfont 0.245 & \fontsize{6.5}{6.5}\selectfont 0.449 \\
            \scriptsize RPMNet (\textit{PPF})~\citep{yew2020rpm} & \fontsize{6.5}{6.5}\selectfont 0.60\textdegree & \fontsize{6.5}{6.5}\selectfont 0.004 & \fontsize{6.5}{6.5}\selectfont 0.005 & \fontsize{6.5}{6.5}\selectfont 16.91\textdegree & \fontsize{6.5}{6.5}\selectfont 0.079 & \fontsize{6.5}{6.5}\selectfont 0.127 \\
            \midrule[0.25pt]
            \scriptsize \OM{} (\textit{RRI})  & \fontsize{6.5}{6.5}\selectfont 0.017\textdegree & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont \textless 0.0001 & \fontsize{6.5}{6.5}\selectfont \textbf{0.053\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{0.0004} & \fontsize{6.5}{6.5}\selectfont \textbf{0.0005} \\
            \scriptsize \OM{} (\textit{FPFH})  & \fontsize{6.5}{6.5}\selectfont \textbf{0.014\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{\textless 0.0001} & \fontsize{6.5}{6.5}\selectfont \textbf{\textless 0.0001} & \fontsize{6.5}{6.5}\selectfont 0.549\textdegree & \fontsize{6.5}{6.5}\selectfont 0.0024 & \fontsize{6.5}{6.5}\selectfont 0.0033  \\
            \scriptsize \OM{} (\textit{PPF})  & \fontsize{6.5}{6.5}\selectfont 0.026\textdegree & \fontsize{6.5}{6.5}\selectfont 0.0002 & \fontsize{6.5}{6.5}\selectfont 0.0002 & \fontsize{6.5}{6.5}\selectfont 0.388\textdegree & \fontsize{6.5}{6.5}\selectfont 0.0024 & \fontsize{6.5}{6.5}\selectfont 0.0030 \\
            \bottomrule[1.2pt]
        \end{tabular}
    \end{center}
    \label{tab:mn40_unseen}
\end{table}

==> table/mn40_unseen_noisy.tex <==
{\setlength{\tabcolsep}{5.5pt}
\begin{table}[]
    % \centering
    \caption{
    \textbf{PPR on ModelNet40 with the ``Unseen \& Noisy'' settings.} 
    $^{\dag}$ denotes ground truth correspondences or cross-contextual information are used during training.
    $NC$ denotes Not-Converge, and it means the network does not converge during training.
    }
    % \vspace{-6mm}
    \begin{center}
    \small{
        \begin{tabular}{l|ccc|ccc}
            % \Xhline{1pt}
            \toprule[1.2pt]
            \multicolumn{1}{c}{} & \multicolumn{3}{c|}{\fontsize{8}{8}\selectfont{[0, 45\text{\textdegree}]}} & \multicolumn{3}{c}{\fontsize{8}{8}\selectfont{[0, 180\text{\textdegree}]}} \\
            % \cline{2-7}
            \cmidrule[0.25pt]{2-7}
            \multicolumn{1}{c}{} & \scriptsize $\mathcal{L}_{\mathbf{R}}$ & \scriptsize $\mathcal{L}_{\mathbf{t}}$ & \scriptsize $\mathcal{L}_{\text{RMSE}}$ & \scriptsize $\mathcal{L}_{\mathbf{R}}$ & \scriptsize $\mathcal{L}_{\mathbf{t}}$ & \scriptsize $\mathcal{L}_{\text{RMSE}}$ \\
            % \hline\hline
            \midrule[0.75pt]
            \scriptsize PRNet$^{\dag}$~\citep{wang2019prnet} &
            \fontsize{6.5}{6.5}\selectfont 8.47\textdegree & \fontsize{6.5}{6.5}\selectfont 0.061 & \fontsize{6.5}{6.5}\selectfont 0.081 & \fontsize{6.5}{6.5}\selectfont $NC$ & \fontsize{6.5}{6.5}\selectfont $NC$ & \fontsize{6.5}{6.5}\selectfont $NC$ \\
            \scriptsize IDAM$^{\dag}$({GNN})~\citep{li2019iterative} & 
            \fontsize{6.5}{6.5}\selectfont 4.25\textdegree & \fontsize{6.5}{6.5}\selectfont 0.025 & \fontsize{6.5}{6.5}\selectfont 0.037 & \fontsize{6.5}{6.5}\selectfont 48.23\textdegree & \fontsize{6.5}{6.5}\selectfont 0.182 & \fontsize{6.5}{6.5}\selectfont 0.333 \\
            \scriptsize IDAM$^{\dag}$(\textit{FPFH})~\citep{li2019iterative} & 
            \fontsize{6.5}{6.5}\selectfont 9.50\textdegree & \fontsize{6.5}{6.5}\selectfont 0.051 & \fontsize{6.5}{6.5}\selectfont 0.087 & \fontsize{6.5}{6.5}\selectfont 66.01\textdegree & \fontsize{6.5}{6.5}\selectfont 0.198 & \fontsize{6.5}{6.5}\selectfont 0.420 \\
             \scriptsize Predator$^{\dag}$~\citep{huang2021predator} & 
            \fontsize{6.5}{6.5}\selectfont 2.91\textdegree & \fontsize{6.5}{6.5}\selectfont 0.017 & \fontsize{6.5}{6.5}\selectfont 0.024 & \fontsize{6.5}{6.5}\selectfont 34.32\textdegree & \fontsize{6.5}{6.5}\selectfont \textbf{0.090} & \fontsize{6.5}{6.5}\selectfont 0.179 \\
            \scriptsize RGM$^{\dag}$~\citep{fu2021robust} & 
            \fontsize{6.5}{6.5}\selectfont 2.62\textdegree & \fontsize{6.5}{6.5}\selectfont 0.025 & \fontsize{6.5}{6.5}\selectfont 0.030 & \fontsize{6.5}{6.5}\selectfont 25.65\textdegree & \fontsize{6.5}{6.5}\selectfont 0.117 & \fontsize{6.5}{6.5}\selectfont 0.179 \\
            % \hline
            \scriptsize DCP~\citep{wang2019deep} &
            \fontsize{6.5}{6.5}\selectfont 10.58\textdegree & \fontsize{6.5}{6.5}\selectfont 0.072 & \fontsize{6.5}{6.5}\selectfont 0.109 & \fontsize{6.5}{6.5}\selectfont 75.34\textdegree & \fontsize{6.5}{6.5}\selectfont 0.192 & \fontsize{6.5}{6.5}\selectfont 0.467 \\
            \scriptsize DeepGMR (\textit{RRI})~\citep{yuan2020deepgmr} & 
            \fontsize{6.5}{6.5}\selectfont 17.67\textdegree & \fontsize{6.5}{6.5}\selectfont 0.067 & \fontsize{6.5}{6.5}\selectfont 0.131 & \fontsize{6.5}{6.5}\selectfont 41.60\textdegree & \fontsize{6.5}{6.5}\selectfont 0.153 & \fontsize{6.5}{6.5}\selectfont 0.308 \\
            \scriptsize DeepGMR (XYZ)~\citep{yuan2020deepgmr} & 
            \fontsize{6.5}{6.5}\selectfont 7.55\textdegree & \fontsize{6.5}{6.5}\selectfont 0.052 & \fontsize{6.5}{6.5}\selectfont 0.071 & \fontsize{6.5}{6.5}\selectfont 70.26\textdegree & \fontsize{6.5}{6.5}\selectfont 0.233 & \fontsize{6.5}{6.5}\selectfont 0.436 \\
            \scriptsize RPMNet~\citep{yew2020rpm} &
            \fontsize{6.5}{6.5}\selectfont 3.80\textdegree & \fontsize{6.5}{6.5}\selectfont 0.022 & \fontsize{6.5}{6.5}\selectfont 0.032 & \fontsize{6.5}{6.5}\selectfont 39.52\textdegree & \fontsize{6.5}{6.5}\selectfont 0.129 & \fontsize{6.5}{6.5}\selectfont 0.271 \\
            % \hline
            \midrule[0.25pt]
            \scriptsize \OM{} (\textit{RRI}) & 
            \fontsize{6.5}{6.5}\selectfont 1.47\textdegree & \fontsize{6.5}{6.5}\selectfont 0.010 & \fontsize{6.5}{6.5}\selectfont 0.012 & \fontsize{6.5}{6.5}\selectfont 51.49\textdegree & \fontsize{6.5}{6.5}\selectfont 0.200 & \fontsize{6.5}{6.5}\selectfont 0.335 \\
            \scriptsize \OM{} (\textit{FPFH}) & 
            \fontsize{6.5}{6.5}\selectfont 1.33\textdegree & \fontsize{6.5}{6.5}\selectfont 0.009 & \fontsize{6.5}{6.5}\selectfont 0.011 & \fontsize{6.5}{6.5}\selectfont 33.21\textdegree & \fontsize{6.5}{6.5}\selectfont 0.140 & \fontsize{6.5}{6.5}\selectfont 0.242 \\
            \scriptsize \OM{} (\textit{PPF}) & 
            \fontsize{6.5}{6.5}\selectfont \textbf{1.12\textdegree} & \fontsize{6.5}{6.5}\selectfont \textbf{0.008} & \fontsize{6.5}{6.5}\selectfont \textbf{0.010} & \fontsize{6.5}{6.5}\selectfont \textbf{21.63\textdegree} & \fontsize{6.5}{6.5}\selectfont {0.111} & \fontsize{6.5}{6.5}\selectfont \textbf{0.169} \\
            % \Xhline{1pt}
            \bottomrule[1.2pt]
        \end{tabular}
        }
    \end{center}
    \label{tab:mn40_unseen_noisy}
\end{table}    
}
